GPU LSM: A Dynamic Dictionary Data Structure for the GPU

We develop a dynamic dictionary data structure for the GPU, supporting fast insertions and deletions, based on the Log Structured Merge tree (LSM). Our implementation on an NVIDIA K40c GPU has an average update (insertion or deletion) rate of 225 M elements/s, 13.5x faster than merging items into a sorted array. The GPU LSM supports the retrieval operations of lookup, count, and range query operations with an average rate of 75 M, 32 M and 23 M queries/s respectively. The trade-off for the dynamic updates is that the sorted array is almost twice as fast on retrievals. We believe that our GPU LSM is the first dynamic general-purpose dictionary data structure for the GPU.

==> cola.tex <==
\section{Preliminaries}\label{sec:cola}\label{sec:prelim}
In this section we briefly discuss the two data structures that form
the basis of our GPU data structure which will be described in
Section~\ref{sec:gpu_cola}.  O'neil et al.~\shortcite{Oneil:1996:LSM}
proposed the LSM-tree as a dictionary data structure suitable for
transactional systems and external memory applications to support
queries while achieving high insertion rates.  \mfc{starting from
  here, things get confusing} The idea was to have multiple
levels of search trees, which are all exponentially scaled, and
changes to each level are batched and cascaded (by merging search
trees) through other levels (potentially on different disk
levels). \mfc{I find this sentence confusing, and I don't know what a
  ``disk level'' is.}

Each sorted array of size $2^k$, for some $k$, is readily equivalent
to a balanced binary search tree.  \mfc{What sorted array?  What does
  ``readily equivalent'' mean?}
By considering an indexed set \mfc{what is an indexed set?} of these
arrays, starting from a singleton and each be doubled in size as its
previous one, we have a skeleton of a data structure that fits into
the LSM-tree model.
All that remains is to define the semantics required for insertions and deletions as well as the machinery behind performing queries.
The \emph{basic} COLA proposed by Bender et al.~\cite{Bender:2007:CSB} is an
amortized dictionary data structure that shares the same skeleton described above.
By ``amortized'' we mean that we can bound the work and depth required
for any sequence of operations, but the work or depth required
for individual operations may vary.
We begin here with a description of a
basic COLA implementation that supports insertions as well as all the
query operations
listed in Section~\ref{sec:dictionaries}, and has a theoretically
sub-optimal query time. \mfc{Can you just borrow the language from the
  COLA paper?  I found this paragraph quite confusing.}

\mfc{Here's an alternative.  Kill everything starting at ``starting
  from here''.

The basic idea of an LSM is to keep a set of dictionaries, each a
constant factor larger than the one before.  As insertions arrive,
they are placed in a small dictionary.  When a dictionary reaches
capacity, it is merged with the next larger dictionary, and so on.

In an LSM, a query must be performed at each level.  Therefore, LSMs
usually have a B-tree at each level.  Since $O(\log n)$ searches must
be performed, the search time in an LSM takes $O(\log n \log_B N)$ I/Os in
the worst case, making them slower for queries than B-trees.  The
improvement comes from the I/Os to insert.  Since items are moved from
one level of the LSM to the next in a batch, the insertions in the
next level can enjoy some locality of reference.  It is possible to
show that LSMs are asymptotically much faster than B-trees for
insertions.

A COLA replaces the B-tree at each level with a sorted array.  This
would seem to make searches slower, since as noted above, B-trees
perform searches faster than binary search into an array.  In the
COLA paper, pointers were maintained between levels via fractional
cascading, through which COLAs enjoy the same search speed as B-trees
while achieving the same insertion complexity as LSM-trees.

Here we do not maintain the inter-level points.  We do use sorted
arrays at each level, because SOMETHING ABOUT THE MAGIC OF GPU
PROGRAMMING GOES HERE.
 }

In a COLA, each level is either completely empty or completely full; see
Figure~\ref{fig:eg_insertion_cola}.
To insert a new element,
we start from the first (smallest) level; let us assume
for simplicity that it has size one.
So either the first level is empty and we insert the new element into it,
or it is already full.
In that case we merge the element in the first level
with the new element to form a sorted array of size two, and attempt to
insert that into the second level.
We continue this procedure
(merge a newly sorted array with an existing sorted level)
until we find an empty level into which we insert our current sorted array.
Hence all levels of the COLA are always sorted.
\textsc{lookup}$(k)$ is performed by a binary search over
all levels.
The \textsc{count}$(k_1,k_2)$ queries similarly can be done with
binary searches for $k_1$ and $k_2$ on every level,
and then calculating the total number of elements in the range using the
indices.
A \textsc{range}$(k_1,k_2)$
query is similar, except we only need a binary search for
$k_1$ on each level, followed listing of subsequent
elements until one larger than $k_2$ is found.
These approaches
have a reasonable but not optimal asymptotic
search time of $O(\lg^2 n)$.

% \paragraph{The GPU LSM}
% What we particularly like about the LSM-trees and the basic COLA is that by their hierarchical (logarithmically scaled) structure they can effectively prevent some parts of the data structure from being touched after each insertion (for example, unlike B-trees).
% We can also implement updates in a consistent way using only two primitives, sort and merge.
% Both sort and merge are bulk primitives that have efficient parallel formulations for GPUs.
% As a result, we would expect to be able to handle high rates of insertions (and deletions) similar to their sequential versions.
% The choice of having a sorted array per level, also gives us a good locality required any high performance GPU program.

% %%%%%%
% The COLA~\cite{Bender:2007:CSB} -- Cache Oblivious Lookahead Array -- is an
% amortized dictionary
% data structure, originally designed for external memory applications.
% By ``amortized'' we mean that we can bound the work and depth required
% for any sequence of operations, but the work or depth required
% for individual operations may vary.
% We begin here with a description of a
% basic COLA implementation that supports insertions as well as all the
% query operations
% listed in Section~\ref{sec:dictionaries}, and has a theoretically
% sub-optimal query time.
% Our full COLA implementation supports deletions as well.
% We discuss the possibility of improving the query time by implementing
% the theoretically optimal query algorithm in
% Section~\ref{sec:conclusion}.

% A COLA consists of an ordered list of sorted arrays,
% known as its \emph{levels}.
% The size of each level is twice the size of its preceding level.
% Each level is either completely empty or completely full; see
% Figure~\ref{fig:eg_insertion_cola}.

% To insert a new element,
% we start from the first (smallest) level; let us assume
% for simplicity that it has size one.
% So either the first level is empty and we insert the new element into it,
% or it is already full.
% In that case we merge the element in the first level
% with the new element to form a sorted array of size two, and attempt to
% insert that into the second level.
% We continue this procedure
% (merge a newly sorted array with an existing sorted level)
% until we find an empty level into which we insert our current sorted array.
% Hence all levels of the COLA are always sorted.

% In this basic COLA, \textsc{lookup}$(k)$ is performed by a binary search over
% all levels.
% The \textsc{count}$(k_1,k_2)$ queries similarly can be done with
% binary searches for $k_1$ and $k_2$ on every level,
% and then calculating the total number of elements in the range using the
% indices.
% A \textsc{range}$(k_1,k_2)$
% query is similar, except we only need a binary search for
% $k_1$ on each level, followed listing of subsequent
% elements until one larger than $k_2$ is found.
% These approaches
% have a reasonable but not optimal asymptotic
% search time of $O(\lg^2 n)$.
% %%%%%%%%%%%%%%%%%
% \subsection{Why COLA?}\label{subsec:why_cola}


% We choose the COLA because we can implement updates in a consistent way using only two primitives, sort and merge.
% Both sort and merge are bulk primitives that have efficient parallel formulations for GPUs.

% %The lack of existing mutable data structures on GPUs emphasizes the challenge in identifying and/or designing a data structure that supports a set of interesting operations with good concurrency and performance while simultaneously allowing mutability.
% We began this project with the following data-structure requirements: 1) support a full set of queries (e.g., lookup, count and range); 2) allow parallel execution of these queries in efficiently exploiting the massive parallelism offered by modern GPUs while guaranteeing correctness at any time; and 3) allow efficient, concurrent mutable insertion and deletion operations (``updates'') at a cheaper cost than completely rebuilding the data structure.
% %Although some GPU data structures focus on a subset of these requirements (with the notable exception of mutability), we are interested in supporting all three.
% We fully expect that a data structure with no support for mutability should outperform one with that support, but we expect that incremental changes to a mutable data structure will be considerably cheaper than an entire rebuild of a non-mutable data structure.

% \nina{Let's cut the following paragraph}
% From the point of view of a highly parallel machine like a GPU, not all approaches to mutability are viable. For instance, a set of updates that must run serially (one update at a time) will likely be uncompetitive. Updates that require locking pieces of the data structure, or require fine- or coarse-grained synchronization to ensure correctness, are significant obstacles to performance and will also likely be uncompetitive. We must instead consider an update strategy that exposes enough concurrency to make full use of the GPU and that respects the principles of efficient GPU programs (e.g., coalesced memory accesses and minimal branch divergence).


% %The basic (serial) COLA also supports the operations we consider from Section~\ref{sec:dictionaries}, except for deletions, which we consider in Section~\ref{subsec:deletion_details}.

